Stability estimate for the broken non-abelian X-ray transform in Minkowski space

We study the broken non-abelian X-ray transform in Minkowski space. This transform acts on the space of Hermitian connections on a causal diamond and is known to be injective up to an infinite-dimensional gauge. We show a stability estimate that takes into account the gauge, leading to a new proof of the transform's injectivity. Our proof leads us to consider a special type of connections that we call light-sink connections. We then show that we can consistently recover a light-sink connection from noisy measurement of its X-ray transform data through Bayesian inversion.

==> Gauge paper/preamble.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

\usepackage[usenames, dvipsnames]{color}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage[hidelinks]{hyperref}
\usepackage{tikz}
\usepackage{xfrac}
\usepackage[super]{nth}

\mathtoolsset{showonlyrefs}

\newcommand{\C}{\mathbb C}
\newcommand{\B}{\mathbb B}
\newcommand{\D}{\mathbb D}
\newcommand{\Q}{\mathbb Q}
\newcommand{\R}{\mathbb R}
\newcommand{\N}{\mathbb N}
\newcommand{\Z}{\mathbb Z}
\newcommand{\PP}{\mathbb P}
\newcommand{\EE}{\mathbb E}
\newcommand{\CX}{\mathcal X}
\newcommand{\CL}{\mathcal L}
\newcommand{\CR}{\mathcal R}
\newcommand{\CU}{\mathcal U}
\newcommand{\CD}{\mathcal D}
\newcommand{\de}{\, \mathrm{d}}
\newcommand{\0}{{\bf 0}}
\newcommand{\1}{{\bf 1}}
\newcommand{\del}{\partial}
\newcommand{\diff}{\mathop{}\!\mathrm{d}}
\newcommand{\pardiff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\der}[2]{\frac{\de #1}{\de #2}}
\newcommand{\norm}[1]{\Vert #1 \Vert}
\newcommand{\abs}[1]{| #1 |}
\newcommand{\dual}[2]{\langle #1 , #2 \rangle}
\newcommand{\one}[1]{\textbf{1}_{#1}}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\eps}{\varepsilon}
\newcommand{\ot}{\leftarrow}

\DeclareMathOperator{\re}{Re}
\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\dbar}{\overline\partial}
\DeclareMathOperator{\intr}{int}
\DeclareMathOperator{\Gr}{Gr}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\eng}{eng}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\area}{area}
\DeclareMathOperator{\per}{per}
\DeclareMathOperator{\dive}{div}
\DeclareMathOperator{\mult}{mult}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\TV}{TV}
\DeclareMathOperator{\Prob}{Prob}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Var}{Var}

\newtheorem{thm}{Theorem}[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{coro}[thm]{Corollary}
\newtheorem{conj}[thm]{Conjecture}

\theoremstyle{definition}
\newtheorem{innercustomthm}{}
\newenvironment{prob}[1]
  {\renewcommand{\theinnercustomthm}{#1}\innercustomthm}
  {\endinnercustomthm}
\newenvironment{solution}
  {\begin{proof}[Solution]\renewcommand{\qedsymbol}{}}
  {\end{proof}}
\newtheorem{defi}[thm]{Definition}
\newtheorem{exc}[thm]{Exercise}
\newtheorem{rem}[thm]{Remark}
\newtheorem{remi}[thm]{Reminder}
\newtheorem{ex}[thm]{Example}
